Recursive Online Enumeration of All Minimal Unsatisfiable Subsets

In various areas of computer science, we deal with a set of constraints to be satisfied. If the constraints cannot be satisfied simultaneously, it is desirable to identify the core problems among them. Such cores are called minimal unsatisfiable subsets (MUSes). The more MUSes are identified, the more information about the conflicts among the constraints is obtained. However, a full enumeration of all MUSes is in general intractable due to the large number (even exponential) of possible conflicts. Moreover, to identify MUSes algorithms must test sets of constraints for their simultaneous satisfiabilty. The type of the test depends on the application domains. The complexity of tests can be extremely high especially for domains like temporal logics, model checking, or SMT. In this paper, we propose a recursive algorithm that identifies MUSes in an online manner (i.e., one by one) and can be terminated at any time. The key feature of our algorithm is that it minimizes the number of satisfiability tests and thus speeds up the computation. The algorithm is applicable to an arbitrary constraint domain and its effectiveness demonstrates itself especially in domains with expensive satisfiability checks. We benchmark our algorithm against state of the art algorithm on Boolean and SMT constraint domains and demonstrate that our algorithm really requires less satisfiability tests and consequently finds more MUSes in given time limits.

==> cube.tex <==
%\documentclass{article}
%\usepackage{tikz}
%\usetikzlibrary{arrows,shapes,positioning}
%
%\begin{document}

\tikzstyle{op}=[opacity=.07]

\begin{tikzpicture}[-,>=stealth',shorten >=1pt,auto,node distance=1cm,minimum size=0.4cm,
thick,every node/.style={draw, ellipse,inner sep=0, outer sep=0},
valid/.style={draw,draw=green},
invalid/.style={dashed,draw,draw=red},
v/.style={fill=green},
i/.style={fill=red}]
\node[valid] (0) []{\tiny 00000};
\node[valid] (01) [above left = 0.8 and -2.5 of 0]{\tiny 10000};
\node[valid] (02) [above left = 0.8 and -1.5 of 0]{\tiny 01000};
\node[valid] (03) [above left = 0.8 and -0.5 of 0]{\tiny 00100};
\node[valid] (04) [above left = 0.8 and 0.5 of 0]{\tiny 00010};
\node[valid] (05) [above left = 0.8 and 1.5 of 0]{\tiny 00001};
\node[valid] (012) [above left = 1.6 and -5.0 of 0]{\tiny 11000};
\node[valid] (013) [above left = 1.6 and -4.0 of 0]{\tiny 10100};
\node[valid] (023) [above left = 1.6 and -3.0 of 0]{\tiny 01100};
\node[valid] (014) [above left = 1.6 and -2.0 of 0]{\tiny 10010};
\node[valid] (024) [above left = 1.6 and -1.0 of 0]{\tiny 01010};
\node[valid] (034) [above left = 1.6 and 0.0 of 0]{\tiny 00110};
\node[invalid] (015) [above left = 1.6 and 1.0 of 0]{\tiny 10001};
\node[invalid] (025) [above left = 1.6 and 2.0 of 0]{\tiny 01001};
\node[valid] (035) [above left = 1.6 and 3.0 of 0]{\tiny 00101};
\node[invalid] (045) [above left = 1.6 and 4.0 of 0]{\tiny 00011};
\node[valid] (0123) [above left = 2.4000000000000004 and -5.0 of 0]{\tiny 11100};
\node[valid] (0124) [above left = 2.4000000000000004 and -4.0 of 0]{\tiny 11010};
\node[valid] (0134) [above left = 2.4000000000000004 and -3.0 of 0]{\tiny 10110};
\node[valid] (0234) [above left = 2.4000000000000004 and -2.0 of 0]{\tiny 01110};
\node[invalid] (0125) [above left = 2.4000000000000004 and -1.0 of 0]{\tiny 11001};
\node[invalid] (0135) [above left = 2.4000000000000004 and 0.0 of 0]{\tiny 10101};
\node[invalid] (0235) [above left = 2.4000000000000004 and 1.0 of 0]{\tiny 01101};
\node[invalid] (0145) [above left = 2.4000000000000004 and 2.0 of 0]{\tiny 10011};
\node[invalid] (0245) [above left = 2.4000000000000004 and 3.0 of 0]{\tiny 01011};
\node[invalid] (0345) [above left = 2.4000000000000004 and 4.0 of 0]{\tiny 00111};
\node[valid] (01234) [above left = 3.2 and -2.5 of 0]{\tiny 11110};
\node[invalid] (01235) [above left = 3.2 and -1.5 of 0]{\tiny 11101};
\node[invalid] (01245) [above left = 3.2 and -0.5 of 0]{\tiny 11011};
\node[invalid] (01345) [above left = 3.2 and 0.5 of 0]{\tiny 10111};
\node[invalid] (02345) [above left = 3.2 and 1.5 of 0]{\tiny 01111};
\node[invalid] (012345) [above left = 4.0 and -0.5 of 0]{\tiny 11111};
\path[every node/.style={font=\sffamily\small}]
(0) edge[op] node [left] {} (01)
    edge[op] node [left] {} (02)
    edge[op] node [left] {} (03)
    edge[op] node [left] {} (04)
    edge[op] node [left] {} (05)
(01) edge[op] node [left] {} (012)
    edge[op] node [left] {} (013)
    edge[op] node [left] {} (014)
    edge[op] node [left] {} (015)
(02) edge[op] node [left] {} (012)
    edge[op] node [left] {} (023)
    edge[op] node [left] {} (024)
    edge[op] node [left] {} (025)
(03) edge[op] node [left] {} (013)
    edge[op] node [left] {} (023)
    edge[op] node [left] {} (034)
    edge[op] node [left] {} (035)
(04) edge[op] node [left] {} (014)
    edge[op] node [left] {} (024)
    edge[op] node [left] {} (034)
    edge[op] node [left] {} (045)
(05) edge[op] node [left] {} (015)
    edge[op] node [left] {} (025)
    edge[op] node [left] {} (035)
    edge[op] node [left] {} (045)
(012) edge[op] node [left] {} (0123)
    edge[op] node [left] {} (0124)
    edge[op] node [left] {} (0125)
(013) edge[op] node [left] {} (0123)
    edge[op] node [left] {} (0134)
    edge[op] node [left] {} (0135)
(023) edge[op] node [left] {} (0123)
    edge[op] node [left] {} (0234)
    edge[op] node [left] {} (0235)
(014) edge[op] node [left] {} (0124)
    edge[op] node [left] {} (0134)
    edge[op] node [left] {} (0145)
(024) edge[op] node [left] {} (0124)
    edge[op] node [left] {} (0234)
    edge[op] node [left] {} (0245)
(034) edge[op] node [left] {} (0134)
    edge[op] node [left] {} (0234)
    edge[op] node [left] {} (0345)
(015) edge[op] node [left] {} (0125)
    edge[op] node [left] {} (0135)
    edge[op] node [left] {} (0145)
(025) edge[op] node [left] {} (0125)
    edge[op] node [left] {} (0235)
    edge[op] node [left] {} (0245)
(035) edge[op] node [left] {} (0135)
    edge[op] node [left] {} (0235)
    edge[op] node [left] {} (0345)
(045) edge[op] node [left] {} (0145)
    edge[op] node [left] {} (0245)
    edge[op] node [left] {} (0345)
(0123) edge[op] node [left] {} (01234)
    edge[op] node [left] {} (01235)
(0124) edge[op] node [left] {} (01234)
    edge[op] node [left] {} (01245)
(0134) edge[op] node [left] {} (01234)
    edge[op] node [left] {} (01345)
(0234) edge[op] node [left] {} (01234)
    edge[op] node [left] {} (02345)
(0125) edge[op] node [left] {} (01235)
    edge[op] node [left] {} (01245)
(0135) edge[op] node [left] {} (01235)
    edge[op] node [left] {} (01345)
(0235) edge[op] node [left] {} (01235)
    edge[op] node [left] {} (02345)
(0145) edge[op] node [left] {} (01245)
    edge[op] node [left] {} (01345)
(0245) edge[op] node [left] {} (01245)
    edge[op] node [left] {} (02345)
(0345) edge[op] node [left] {} (01345)
    edge[op] node [left] {} (02345)
(01234) edge[op] node [left] {} (012345)
(01235) edge[op] node [left] {} (012345)
(01245) edge[op] node [left] {} (012345)
(01345) edge[op] node [left] {} (012345)
(02345) edge[op] node [left] {} (012345)
;
\end{tikzpicture}
%\end{document}

==> hypercube.tex <==
%\documentclass{article}
%\usepackage{tikz}
%\usetikzlibrary{arrows,shapes,positioning}

%\usepackage[a4paper, total={7in, 8in}]{geometry}

%\begin{document}

\begin{tikzpicture}[-,>=stealth', shorten >=1pt,auto,node distance=1.6cm,minimum size=0.3cm,
  thick,every node/.style={draw=none,inner sep=0, outer sep=0, scale=1.2},invalid/.style={circle,dashed,draw}]

\node[] (0) {$\scriptstyle\emptyset$};

\node[] (2) [above left = 0.4cm and 0.45cm of 0] {$\scriptstyle\{\varphi_2\}$};
\node[] (1) [left of=2] {$\scriptstyle\{\varphi_1\}$};
\node[] (3) [right of=2] {$\scriptstyle\{\varphi_3\}$};
\node[] (4) [right of=3] {$\scriptstyle\{\varphi_4\}$};

\node[] (12) [above left = 0.4cm and 0.35cm of 1] {$\scriptstyle\{\varphi_1,\varphi_2\}$};
\node[] (13) [right = 0.5cm of 12] {$\scriptstyle\{\varphi_1,\varphi_3\}$};
\node[] (14) [right = 0.5cm of 13] {$\scriptstyle\{\varphi_1,\varphi_4\}$};
\node[] (23) [right = 0.5cm of 14] {$\scriptstyle\{\varphi_2,\varphi_3\}$};
\node[] (24) [right = 0.5cm of 23] {$\scriptstyle\{\varphi_2,\varphi_4\}$};
\node[] (34) [right = 0.5cm of 24] {$\scriptstyle\{\varphi_3,\varphi_4\}$};

\node[draw,inner sep=0.1cm] (123) [above right = 0.4cm and -1.22cm of 12] {$\scriptstyle\{\varphi_1,\varphi_2,\varphi_3\}$};
\node[draw,inner sep=0.1cm] (124) [right = 0.7cm of 123] {$\scriptstyle\{\varphi_1,\varphi_2,\varphi_4\}$};
\node[draw,inner sep=0.1cm] (134) [right = 0.7cm of 124] {$\scriptstyle\{\varphi_1,\varphi_3,\varphi_4\}$};
\node[draw,dashed, inner sep=0.1cm] (234) [right = 0.7cm of 134] {$\scriptstyle\{\varphi_2,\varphi_3,\varphi_4\}$};

\node[] (1234) [above right = 0.4cm and -0.75cm of 124] {$\scriptstyle\{ \varphi_1,\varphi_2,\varphi_3,\varphi_4 \}$};

\path[every node/.style={font=\sffamily\small},line width=0.5pt]
(0) 	edge node [left,thin, dashed] {} (1)
		edge node [left] {} (2)
		edge node [left] {} (3)
		edge node [left] {} (4)
(1) 	edge node [left] {} (12)
		edge node [left] {} (13)
		edge node [left] {} (14)
(2) 	edge node [left] {} (12)
		edge node [left] {} (23)
		edge node [left] {} (24)
(3) 	edge node [left] {} (13)
		edge node [left] {} (23)
		edge node [left] {} (34)
(4) 	edge node [left] {} (14)
		edge node [left] {} (24)
		edge node [left] {} (34)
		
(12) 	edge node [left] {} (123)
		edge node [left] {} (124)
(13) 	edge node [left] {} (123)
		edge node [left] {} (134)
(14) 	edge node [left] {} (124)
		edge node [left] {} (134)
(23) 	edge node [left] {} (123)
		edge node [left] {} (234)	
(24) 	edge node [left] {} (124)
		edge node [left] {} (234)
(34) 	edge node [left] {} (134)
		edge node [left] {} (234)
		
(123) 	edge node [left] {} (1234)
(124) 	edge node [left] {} (1234)
(134) 	edge node [left] {} (1234)
(234) 	edge node [left] {} (1234)																	
;

\end{tikzpicture}


%\end{document}

